Physical Attacks on the Railway System

Recent attacks encouraged public interest in physical security for railways. Knowing about and learning from previous attacks is necessary to secure against them. This paper presents a structured data set of physical attacks against railways. We analyze the data regarding the used means, the railway system's target component, the attacker type, and the geographical distribution of attacks. The results indicate a growing heterogeneity of observed attacks in the recent decade compared to the previous decades and centuries, making protecting railways more complex.

==> minutes/Structure.tex <==
Working title: Key target points of the railway system: a review of physical attacks 
Organisation for  http://sam.udmercy.edu/sam23

 Abstract
The railway system is a critical infrastructure for nowadays societies. In the same way, it is one of its key vulnerabilities. This paper reviews xxx physical attacks to the railway system worldwide and assesses what parts of the railway system have been primarily targeted, with which aims and tools. 
We provide an open dataset, but look at the data. 
What is the key target in the railway systems? What countries are prone to attacks? What methods are used? What groups are relevant? Information about the country  how many attacks are per country (DZSF)

\textbf{Friday 17.02  }
    •	Division of work
    •	Organisation of the analysis and agreement on the schedule
    •	Updates from DZSD
    •	Send table of the attacks (UniBw to DZSF)
    
\textbf{M 20.02
}    •	DZSF and UniBW: gathering sources and writing background information – relevance of railway as CI
    •	Categories ready for the database (UNIBW feedback by 23.02)
    
\textbf{M 27.02}
•	DZSF and UniBW: gathering sources and writing background information 
•	DZSF: analysis of the data (students)

\textbf{M 06.03}
        •	DZSF: writing key results
        •	DZSF and UniBW: meeting for discussing key results and conclusions: having this information in bullet points so that UNIBW extends it into text
        
\textbf{M 13.03} 
    •	UniBW: writing of key results and conclusions
    	\textbf{UniBW: Preliminary draft – Prof. Pickl, Prof. Lehnert}
    
\textbf{M 20.03}
    •	First review of the paper and comments (DZSF)
    
\textbf{M 27.03} 
    •	Second review of the paper and comments (UniBW)
    
\textbf{M 03.04}
    •	External feedback, authors: Mr Schmitz, Mr Neubecker, Prof. Pickl
    •	Formalities
    •	EBA Press Office (at the beginning of the week)
    
\textbf{M 10.04}
\textbf{ Wednesday 12.4.2023 Submission of full paper – 7 pages}

